Extension of HOPS Out to 500 ParSecs (eHOPS). I. Identification and Modeling of Protostars in the Aquila Molecular Clouds

We present a Spitzer/Herschel focused survey of the Aquila molecular clouds ($d \sim 436$~pc) as part of the eHOPS (extension of HOPS Out to 500 ParSecs) census of nearby protostars. For every source detected in the Herschel/PACS bands, the eHOPS-Aquila catalog contains 1-850~$\mu$m SEDs assembled from 2MASS, Spitzer, Herschel, WISE, and JCMT/SCUBA-2 data. Using a newly developed set of criteria, we classify objects by their SEDs as protostars, pre-ms sequence stars with disks, and galaxies. A total of 172 protostars are found in Aquila, tightly concentrated in the molecular filaments that thread the clouds. Of these, 71 (42\%) are Class 0 protostars, 54 (31\%) are Class I protostars, 43 (25\%) are flat-spectrum protostars, and 4 (2\%) are Class II sources. Ten of the Class 0 protostars are young PACS Bright Red Sources similar to those discovered in Orion. We compare the SEDs to a grid of radiative transfer models to constrain the luminosities, envelope densities, and envelope masses of the protostars. A comparison of the eHOPS-Aquila to the HOPS protostars in Orion finds that the protostellar luminosity functions in the two star-forming regions are statistically indistinguishable, the bolometric temperatures/envelope masses of eHOPS-Aquila protostars are shifted to cooler temperatures/higher masses, and the eHOPS-Aquila protostars do not show the decline in luminosity with evolution found in Orion. We briefly discuss whether these differences are due to biases between the samples, diverging star formation histories, or the influence of environment on protostellar evolution.

==> pacs_obs.tex <==
\begin{deluxetable*}{cccccc} 
\tablecaption{Observation details for Herschel/PACS \label{tab:pacs}} 
\centering 
\tablehead{ 
\colhead{Wavelength} & \colhead{Observation ID} & \colhead{R.A.} & \colhead{Decl.} & \colhead{Proposal} & 
\colhead{Scan Velocity} \\ 
\colhead{($\micron$)} & \nocolhead{} & \colhead{($\deg$)} & \colhead{($\deg$)} & \nocolhead{} & 
\colhead{($\arcsec$/sec)} 
} 
\decimalcolnumbers 
\startdata 
70 & 1342186277,1342186278 & 277.6 & -2.73 & SDP\_pandre\_3 & 60 \\ 
70 & 1342206676,1342206695 & 277.77 & 0.72 & KPGT\_pandre\_1 & 60 \\ 
70 & 1342206694,1342206696 & 280.01 & 0.05 & KPGT\_pandre\_1 & 60 \\ 
100 & 1342228960,1342228961 & 279.46 & -1.3 & KPGT\_pandre\_1 & 20 \\ 
100 & 1342229079,1342229080 & 277.45 & 0.89 & KPGT\_pandre\_1 & 20 \\ 
100 & 1342193534,1342193535 & 277.83 & -2.09 & KPGT\_pandre\_1 & 20 \\ 
100 & 1342206702,1342206703 & 277.08 & -3.63 & KPGT\_pandre\_1 & 20 \\ 
160 & 1342228960,1342228961 & 279.46 & -1.3 & KPGT\_pandre\_1 & 20 \\ 
160 & 1342193534,1342193535 & 277.83 & -2.09 & KPGT\_pandre\_1 & 20 \\ 
160 & 1342206676,1342206695 & 277.77 & 0.69 & KPGT\_pandre\_1 & 60 \\ 
160 & 1342206702,1342206703 & 277.08 & -3.63 & KPGT\_pandre\_1 & 20 \\ 
160 & 1342186277,1342186278 & 277.59 & -2.73 & SDP\_pandre\_3 & 60 \\ 
160 & 1342206694,1342206696 & 280.01 & 0.05 & KPGT\_pandre\_1 & 60 \\ 
160 & 1342229079,1342229080 & 277.45 & 0.89 & KPGT\_pandre\_1 & 20 \\ 
\enddata 
\tablecomments{We use Level 2.5 processed Herschel/PACS observations that are selected from JSCANAM data products.} 
\end{deluxetable*} 

